Limits on Gradient Compression for Stochastic Optimization

We consider stochastic optimization over $\ell_p$ spaces using access to a first-order oracle. We ask: {What is the minimum precision required for oracle outputs to retain the unrestricted convergence rates?} We characterize this precision for every $p\geq 1$ by deriving information theoretic lower bounds and by providing quantizers that (almost) achieve these lower bounds. Our quantizers are new and easy to implement. In particular, our results are exact for $p=2$ and $p=\infty$, showing the minimum precision needed in these settings are $\Theta(d)$ and $\Theta(\log d)$, respectively. The latter result is surprising since recovering the gradient vector will require $\Omega(d)$ bits.

==> abstract.tex <==
\begin{abstract}
  We consider stochastic optimization over $\ell_p$ spaces using
  access to a first-order oracle.  We ask: {What is the minimum
    precision required for oracle outputs to retain the unrestricted
    convergence rates?}  We characterize this precision for every
  $p\geq 1$ by deriving information theoretic lower bounds and by
  providing quantizers that (almost) achieve these lower bounds.  Our
  quantizers are new and easy to implement.  In particular, our
  results are exact for $p=2$ and $p=\infty$, showing the minimum
  precision needed in these settings are $\Theta(d)$ and $\Theta(\log
  d)$, respectively. The latter result is surprising since recovering
  the gradient vector will require $\Omega(d)$ bits.
\end{abstract}



